RITA: Group Attention is All You Need for Timeseries Analytics

Timeseries analytics is of great importance in many real-world applications. Recently, the Transformer model, popular in natural language processing, has been leveraged to learn high quality feature embeddings from timeseries, core to the performance of various timeseries analytics tasks. However, the quadratic time and space complexities limit Transformers' scalability, especially for long timeseries. To address these issues, we develop a timeseries analytics tool, RITA, which uses a novel attention mechanism, named group attention, to address this scalability issue. Group attention dynamically clusters the objects based on their similarity into a small number of groups and approximately computes the attention at the coarse group granularity. It thus significantly reduces the time and space complexity, yet provides a theoretical guarantee on the quality of the computed attention. The dynamic scheduler of RITA continuously adapts the number of groups and the batch size in the training process, ensuring group attention always uses the fewest groups needed to meet the approximation quality requirement. Extensive experiments on various timeseries datasets and analytics tasks demonstrate that RITA outperforms the state-of-the-art in accuracy and is significantly faster -- with speedups of up to 63X.

==> 3transformer_for_time_series.tex <==
\section{\system: Transformer for Timeseries}
\label{sec.rita}
In this section, we first introduce the overall \system approach. We then show how to use \system to support various downstream tasks. 

%Our goal is to develop a tool for general time series analytics tasks, not limited in generative task like time series prediction. With the feature extracted by Encoder, we can do classification/clustering on the global feature of time series; and do prediction/imputation/outliner detection on the local feature of target parts of time series.
\begin{sloppypar}

\subsection{The \system Encoder}
\label{sec.rita.encoder}

\subsubsection{The Overview\nopunct}\ \\
\noindent\textbf{The Key Idea.} \system leverages the Transformer Encoder~\cite{DBLP:conf/nips/VaswaniSPUJGKP17}. The Decoder in the Transformer is not used, because it is for generative tasks solely such as translation in NLP. In particular, each input sample of Transformer Encoder $\mathbf{X} \in \mathbb{R}^{n*d}$ represents the embeddings of $n$ semantic units (i.e. $n$ word embedding in NLP). Each embedding has $d$ dimensions. Then Encoder models the correlations between these semantic units and outputs $\mathbf{Y} \in \mathbb{R}^{n*d}$ as the context-aware embedding of these $n$ semantic units.

To fill the gap between timeseries and natural language, \system uses a {\bf time-aware convolution} strategy which chunks one input timeseries into $n$ windows and automatically produces one embedding per window. These embeddings are then fed into the Transformer Encoder as its input, as shown in Fig.~\ref{fig.convolution}.
The intuition is that timeseries are typically composed of a set of local patterns which have independent meanings and hence can be treated as the semantic units like words in natural language. For example, these patterns might represent cyber-security breaches, occurrences of seizures, or selling or buying opportunities in stock market.  

Inspired by the success of CNNs in computer vision tasks, which use {\it convolution} to capture the local structures in each image patch, we leverage convolution to capture the local patterns in timeseries. Treating a multi-channel timeseries as a matrix where each row represents one channel and each column corresponds to one timestamp and conducting a convolution operation on it, \system automatically discovers the correlations across different channels, thus naturally solving the multi-channel problem.


\begin{figure}[t]
%\vspace{-3mm}
    \centering
    \includegraphics[width=1.0\columnwidth]{figures/rita_conv.pdf}
    \vspace{-5mm}
    \caption{Convolution in \system}
    \label{fig.convolution}
    \vspace{-6mm}
\end{figure}

\subsubsection{Technical Details\nopunct}\ \\
%\vspace{-1mm}
\noindent\textbf{Input Embedding.}
We denote a raw timeseries as $T \in \mathbb{R}^{t*m}$, which corresponds to a multi-channel (multivariate) timeseries of length $t$ with $m$ channels (variables). The input embedding $X$ to Transformer Encoder is generated by:
\vspace{-1mm}
\begin{equation}
\label{eq.convolution}
X_{i,j}=\sum_{k=0}^m  \sum_{l=0}^{KernelSize}W_{j,k,l}*T_{i+l,k}+ B_{j,k} 
\end{equation}

%\lei{Introduce in more details how convolution works. For example, what is a convolution kernel? what does d, m, kernelSize stand for? Convolution kernel is learned jointly with the transformer encoder, etc. Ideally, explain it with an example here. }

In Eq.~\ref{eq.convolution}, $B \in \mathbb{R}^{d*m}$ is bias. $W$ $\in$ $\mathbb{R}^{d \times m \times KernelSize}$ corresponds to the weight of the convolution layer, where $d$ represents the number of the convolution kernels and $m \times KernelSize$ defines one convolution kernel as a $m \times KernelSize$ matrix. The convolution kernel has $m$ rows, each corresponding to one channel of the timeseries. KernelSize defines the number of timestamps that each convolution kernel covers, identical to the window size in sliding window.  

The convolution kernel slides from left to right on the timeseries matrix over the time axis and computes the dot product with the corresponding timeseries sub-matrix covered by each window. In this way it produces one value for each window;  this value is the feature of this window. 
Because the convolution layer uses $d$ convolution kernels, it produces a $d$-dimensional feature embedding for each window. In Eq.~\ref{eq.convolution}, $X_{i,j}$ stands for the $j$th dimension of the embedding produced for the $i^{th}$ window.
Note the convolution kernels are learned jointly with the Transformer encoder. 

\noindent\textbf{Position Embeddings.}
As mentioned before, temporal order is important in timeseries analytics. We thus use position embedding to make \system aware of the time ordering among the local embeddings extracted by convolution. 
In addition, a special embedding vector \textbf{[CLS]} is attached at the start of input, serving as a global information aggregator.  
To be specific, input $Z$ is generated by $\mathit{Z=[CLS] \textcircled{+} (X+P)}$, where $\mathit{P=[p_1,p_2,...,p_n]}$, $p_i$ $\in$ $\mathbb{R}^d$ is the embedding of position $i$ and \textcircled{+} denotes concatenation. 
As is widely adopted in NLP, we use learnable position embedding~\cite{DBLP:conf/naacl/DevlinCLT19}, which means all $p_i$ are trainable parameters. 
%%try batch norm

\subsection{Downstream Tasks}
\label{sec.transformer.downstream}

The \system Encoder supports a variety of downstream tasks, as shown in Fig.~\ref{fig.overview}. In this section, we show that with minimal modification \system encoder is able to effectively support classification, imputation and forecasting tasks. 
Other unsupervised analytics tasks such as similarity search or clustering are naturally supported by extracting feature embeddings from \system encoder.

\subsubsection{Classification\nopunct}\ \\
Timeseries classification is of great importance in many real-world applications, such as human activity recognition(HAR) and disease diagnosis on electrocardiogram data.

To classify timeseries, we input timeseries to the model as described in Sec.~\ref{sec.rita.encoder}, and feed the output representation of \textbf{[CLS]} into a classifier: $\mathit{y=Softmax(W_{cls}Z_{[CLS]}+B_{cls})}$, where $Z_{[CLS]}\in \mathbb{R}^d$ is the output representation of \textbf{[CLS]}, C is the number of classes, and $\mathit{W_{cls} \in \mathbb{R}^{C \times d}, B_{cls} \in \mathbb{R}^{C}}$ are learnable parameters for classification task. 
The result vector $y\in \mathbb{R}^{C}$ represents the possibility that the input timeseries belongs to each class.

We apply Cross Entropy Loss as the loss function of the classification task~\cite{cox1958regression}:
$\mathit{L=\frac{1}{C}\sum_{i=1}^C -\hat{y}(i)log(y(i))}$, where $\hat{y}$ is a binary indicator for ground truth label:
\vspace{-1mm}
\begin{eqnarray}
\hat{y}(i) =
\begin{cases}
1   & i\  \text{is ground truth label} \\
0   & otherwise
\end{cases}
\end{eqnarray}

%or replaced with reasonable values
\subsubsection{Imputation\nopunct}\ \\
\label{sec.transformer.imputation}
Timeseries are mainly generated by sensors, a common problem of which is missing values. This becomes a challenge when many downstream analytics require the missing values to be recovered. The recovering task is imputation. 

Denote the real timeseries as $T_{r} \in \mathbb{R}^{n \times c}$, the observed timeseries with missing values as $T_{o} \in \mathbb{R}^{n \times c}$, and the set of missing values' positions as $M$. We scale the values of all timeseries to non-negative and use a special value (-1) to indicate missing values:
\vspace{-1mm}
\begin{eqnarray}
\label{eq.imp_task}
T_{o}(i,j) =
\begin{cases}
-1   & (i,j) \in M\\
T_{r}(i,j)   & (i,j) \notin M \\
\end{cases}
\end{eqnarray}

The observed timeseries is fed into the \system Encoder model as input, and the output representations are concatenated and fed into a {\it Transpose Convolution} layer which decodes the output embedding vectors from hidden space to timeseries values, corresponding to the convolution operation in the input stage, i.e., 
$\mathit{Y=TransposeCNN(Z_1 \textcircled{+} Z_2 \textcircled{+} ... \textcircled{+} Z_n)}$, where $Y \in \mathbb{R}^{n \times c}$ is the recovered timeseries, and $Z_i \in \mathbb{R}^d$ is the output of each position.

Here Mean Square Error is chosen as the loss function~\cite{thompson1990mse}:
$L=\frac{1}{|M|}\sum_{(i,j) \in M} (Y(i,j)-T_{r}(i,j))^2$.

\vspace{-2mm}
\subsubsection{Forecasting\nopunct}\ \\
%\vspace{-0.5mm}
In many domains such as economics and finance, forecasting timeseries' future trends is critical~\cite{atsalakis2011elliott,wang2012stock,pai2005hybrid}. Forecasting can be regarded as a special case of imputation, in which all missing values are at the end of timeseries. 
Due to the space limit, please refer to our technical report~\cite{RITA} for the details.

\vspace{-2mm}
\subsubsection{Other Unsupervised Tasks\nopunct}\ \\
%\vspace{-0.5mm}
Other unsupervised tasks, such as similarity search and clustering, are important tools for exploring timeseries databases~\cite{lin1995fast,keogh2001dimensionality,liao2005clustering}, including discovering stocks with similar price trends, finding patience with similar EEG patterns, etc.

\system naturally supports these tasks by producing for the timeseries objects feature embeddings that better reflect their semantic similarity. The embedding of one timeseries corresponds to the output representation of the special token \textbf{[CLS]}, discussed in Sec~\ref{sec.rita.encoder}.
Clustering can be performed on the embeddings with flexible choice of distance metrics. Similarly, a high dimensional similarity search system~\cite{johnson2019billion, malkov2018efficient, jegou2010product} can be built on the embeddings. 

\begin{comment}
So like in imputation task, we scale the timeseries to non-negative and use a special value (-1) to indicate the values to be predicted:
\begin{eqnarray}
T_{observed}(i,j) =
\begin{cases}
T_{real}(i,j)   & i \leq t_{observed} \\
-1   & otherwise
\end{cases}
\end{eqnarray}

Where $t_{observed}$ is the observed timestamp. Then the output representations are fed into a Transpose Convolution layer using Mean Squared Error as loss function, as described above.
\end{comment}

\vspace{-2mm}
\subsection{Self-supervised Pretraining}
\label{sec.transformer.pretraining}
Inspired by the ``cloze text'' pretraining task in NLP, we designed a mask-and-predict task as the pretraining task for our model. The timeseries is randomly masked and the model should recover the masked values based on corresponding contextual information.

As described before, timeseries is not language. We thus use convolution to transform a timeseries into a sequence of windows and produce an input feature embedding per window. However, although \system learns feature embedding at window level, unlike the traditional pretraining in NLP which replaces the embeddings of a masked word with a special predefined embedding, it conducts masking on the {\it raw} timeseries. That is, we replace the values in raw timeseries and let \system recover these values, which can be regarded as denoising autoregression~\cite{vincent2010stacked}.
%can not simply replace the embedding of a masked word with a special predefined embedding like in

To be specific, we generate masks on time-stamps, with an expected mask rate $p$. The timeseries is scaled to be non-negative and the values across all the channels on the masked timestamps are set to be -1, an impossible value on normal timestamps. Then the masked timeseries is fed into \system encoder and the output representation is translated to the recovered timeseries by a Transpose Convolution layer, as described in the imputation task (Sec.~\ref{sec.transformer.imputation}).

Pretraining encourages \system to learn the dependencies across different channels over time. Meanwhile, pretraining on unlabeled timeseries gives the model a prior knowledge of data distribution of the corresponding domain, thus mitigating the issue of overfitting when training with few labeled data on downstream tasks.
\end{sloppypar}















==> discussion.tex <==
\section{Discussion}
\label{sec.discussion}
\jm{added}
In this work, we presented \system, an automatic, self-supervised, and scalable timeseries analytics tool. \system effectively adapts Transformer, popular in NLP, into timeseries analytics. 
As the key component of \system,  group attention  eliminates the performance bottleneck of the classical self-attention mechanisms, thus successfully scaling \system to highly complex, long timeseries data.
Our experiments confirm that \system significantly speeds up the state-of-the-art by 63X with a better accuracy. 
%\srm{Say how much better - give concrete numbers.}

==> introduction-backup.tex <==
%\vspace{-3mm}
\section{Introduction}
\label{sec.intro}
\noindent\textbf{Motivation.} Many data driven applications involve processing massive timeseries data, including IoT~\cite{cook2019anomaly}, medical AI~\cite{crabtree1990individual}, stock market~\cite{kraft1977determinants}, bank transactions~\cite{soro2020regular}, and so on. As such, there is a great need for timeseries analytics, such as trend recognition~\cite{shimakawa1992trend}, forecasting~\cite{chatfield2000time}, classification~\cite{ismail2019deep}, clustering~\cite{liao2005clustering}, similarity search~\cite{negi2005time}, and anomaly detection~\cite{teng2010anomaly}, with application ranging from identifying device failure~\cite{sun2019system}, automatically diagnosing diseases~\cite{bui2017time}, recognizing human activities~\cite{lara2012survey}, to stopping financial fraud~\cite{yue2007review}. 

To date, applications still mainly use traditional techniques such as ARIMA~\cite{arima}, TS-CHIEF~\cite{Shifaz2020TSCHIEFAS}, HIVE-COTE~\cite{10.1145/3182382}, and ROCKET~\cite{DBLP:journals/datamine/DempsterPW20}, to analyze timeseries data, which either heavily rely on humans to manually extract features based on their domain knowledge or are inadequate in handling complex multi-variate timeseries data.

A natural question is to ask whether deep learning -- which has revolutionized domains such as computer vision and natural language processing (NLP) -- could be applied.
To date, however, attempts to apply it to timeseries~\cite{DBLP:conf/kdd/ZerveasJPBE21} have not shown it to be universally superior, because deep learning requires extensive labeled examples and massive computational power to be effective.
In particular, despite the abundance of timeseries data in this ``Big Data'' era, the availability of labeled data is far more limited: extensive data labeling is often prohibitively expensive, as it typically requires a great deal of time and effort from domain experts.  

% \begin{figure}{}
% \vspace{-2mm}
%     \centering
%     \includegraphics[width=1.0\columnwidth]{figures/overview.pdf}
%     \vspace{-7mm}
%     \caption{Overview of \system}
%     \label{fig.overview}
%     \vspace{-8mm}
% \end{figure}

%\vspace{-3mm}
\noindent\textbf{The \system Strategy.} 
We propose to tackle the aforementioned problems by building a general-purpose timeseries analytics tool that is {\bf automatic} -- freeing humans from manual feature extraction, {\bf self-supervised} -- requiring no labels while offering high accuracy by leveraging the existing plethora of unlabeled data, and {\bf scalable} -- efficiently handling highly complex, massive-scale timeseries data. 

The key observation is that in timeseries data, the sequential order among the values (stock trading price, volume, etc.) over time matters. That is, each value is highly correlated with other values observed before or after it. 
This fundamental property of timeseries bears similarity to natural language at a high level, where a word is correlated to other words in each sentence.  
Inspired by the {\it mask and predict} methodology used in Bert~\cite{DBLP:conf/naacl/DevlinCLT19} which has been remarkably successful in natural language processing (NLP)~\cite{DBLP:conf/naacl/DevlinCLT19}, we developed a {\it self-supervised} pre-training method, called \system, to train a deep learning model which takes the correlations among different observations into consideration. 

%Fig.~\ref{fig.overview} shows an overview of \system. 
Given a collection of {\it unlabeled} timeseries, \system first pre-trains a Transformer model which {\it automatically} produces high quality feature embeddings for timeseries data. This pre-trained model are then used to support various downstream tasks. For example, as with BERT, \system supports {\it supervised tasks} such as classification by fine-tuning the pre-trained parameters to achieve high accuracy with {\it small number} of labels.
\system also naturally supports other {\it analytics} tasks such as forecasting, missing value imputation, and outlier detection. \system automatically produces feature embeddings by randomly masking some of the values from the input timeseries and predicting the masked values based on their contexts. It thus can be used to directly impute missing values and future values, while outliers can be identified as the observations that significantly deviate from their corresponding predictions~\cite{10.1007/978-3-030-77964-1_17}. {\it Unsupervised analytics tasks} such as clustering and similarity search can run directly on the feature embeddings produced by \system, which encode the long term trends of the timeseries and tend to be more informative than the raw features traditionally used in modeling the similarity of different timeseries objects~\cite{DBLP:conf/kdd/WangP21}.

%\vspace{-3mm}
\noindent\textbf{Scalability Challenge.} The key challenge is to make \system scalable to long timeseries.
The idea of self-attention~\cite{DBLP:conf/nips/VaswaniSPUJGKP17} is central to pre-training methods in NLP. Self-attention computes the pairwise correlations among different semantic units in a sentence, and as such, has {\it quadratic} time and space complexity in the length of the input sequence. 
This limits the model's scalability, especially when handling large-scale timeseries data, which is common in real-world applications such as IoT, medical AI, and finance~\cite{zhou2021informer,DBLP:journals/pvldb/CaoTAJYLGSBSCWM19,liu2018open}. Predictions about timeseries may need to look at months or years of historical data to make accurate predictions, spanning hundreds of thousands of samples.  
As a concrete example, in collaboration with a research hospital we have been developing a seizure classifier~\cite{DBLP:journals/pvldb/CaoTAJYLGSBSCWM19} that automatically detects seizures based on EEG signals (timeseries) collected during the clinical observation of patients. As seizures last only a few seconds, we chunk long EEG data into many 2 second segments and detect seizures at a segment level. However, the classification of a particular segment depends on up to 12 hours of prior signal to determine if one 2 second segment indicates seizure or not, because seizure diagnosis needs to consider the long-term trend of the EEG data. The number of segments in 12 hours is more than 21k. 
This is far larger than the number of semantic units the typical NLP tasks expect. For example, BERT~\cite{DBLP:conf/naacl/DevlinCLT19} limits the number of units to 512 \srm{and even massive models like GPT-3 limit the number of units to XXX}.
Existing works~\cite{DBLP:conf/kdd/ZerveasJPBE21} directly apply Transformers to process timeseries data and thus are not scalable to such long inputs. 
Although in NLP some lower complexity methods have been proposed to {\it approximately} compute self-attention~\cite{kitaev2020reformer,choromanski2020rethinking,wang2020linformer}, their performance degrades dramatically when used on timeseries due to the gap between natural language and timeseries, as shown in our experiments. 

%This is far more than the number of semantic units the typical NLP tasks expect. For example, GPT-3, which took tens of years of GPU time to train, limits the number of units to 2048.
%\vspace{-3mm}
\noindent\textbf{Proposed Approach.} 
To scale \system to long timeseries, we  propose a novel attention mechanism, called {\bf group attention}. Leveraging the periodicity of timeseries, \system chunks the timeseries into segments and dynamically clusters the segments of each input timeseries into a small number of groups, where the segments in the same group have similar feature embeddings during the current training iteration and thus can share the attention computation. The longer the timeseries is, the more sharing opportunities it offers.
\system then computes the self-attention at the group level.
In this way, group attention produces a {\it compressed attention matrix} and eliminates both the CPU and memory bottleneck in transformer-style models, thus scalable to long timeseries.

Moreover, to preserve the accuracy on the downstream tasks, we design an {\it embedding aggregation} strategy and a customized {\it group softmax function} which together ensure \system is still able to produce high quality feature embeddings using this compressed attention matrix. 
We design GPU friendly strategy to group the segments {\it in parallel}, effectively minimizing the grouping overhead.

\textbf{Adaptive Scheduling.}
In \system, {\it the number of groups} $N$ balances the speed up and the quality of attention approximation. A small $N$ will lead to a large speed up, but potentially large approximation errors. On the other hand, although a large $N$ tends to produce high-quality approximations, it inevitably slows down the training process. Therefore, an appropriate $N$ is critical to the performance of group attention. However, $N$ depends on the distributional properties of the datasets. Furthermore, like the classical transformer models, \system stacks multiple attention layers to produce better embeddings. Different layers should also use different values of $N$. 
This makes manually setting an appropriate $N$ almost impossible. 

To solve this problem, we propose an adaptive scheduling strategy which dynamically decides an appropriate $N$ in the training process. It starts with a large $N$ and iteratively merges groups that are similar to each other. Guided by an error bound on the approximated self-attention that users can tolerate, it automatically determines if two groups are mergeable, performing merging efficiently in a GPU-friendly way. 

\textbf{Batch Size.} As \system adjusts $N$ dynamically during training, a fixed batch size raises problems: as $N$ decreases, the memory usage of a single sample decreases. This allows a larger batch size which is beneficial, because: 
(1) it makes full use of GPU memory; (2) high-parallelism across the samples in a big batch brings better performance. 
Our experimental study shows that doubling the batch size reduces the training time by 30\%, while still preserving the quality of the model. Thus, \system should dynamically adjust batch-size as $N$ changes.

We thus propose a learning-based method to model the correlation between the number of groups $N$ and the batch size $B$. The model is then used to predict $B$ for a given $N$ when training \system.
More specifically, we first sample some $N$ values in a reasonable range. For each sampled $N$, we find a batch size that consumes up to a certain percentage of GPU memory in a cost-efficient way. Using a small set of mathematical functions as prior, \system learns the model with only a few <N, B> pairs as ground truth labels.    

Our experiments on public timeseries benchmarks and the MGH EEG data~\cite{DBLP:journals/pvldb/CaoTAJYLGSBSCWM19} confirm that \system outperforms the state-of-the-art methods in accuracy on various timeseries analytics tasks, while our group attention mechanism achieves a 63X speedup with much less memory required, compared to the existing self-attention mechanisms~\cite{DBLP:conf/nips/VaswaniSPUJGKP17,choromanski2020rethinking,wang2020linformer}.

\noindent\textbf{Contributions.} The key contributions of this work include:

\begin{compactitem}
\item We build \system, a general-purpose timeseries analytics tool that is automatic, self-supervised, scalable to high complexity, massive-scale timeseries data.

% \item We design a time-aware convolution operation to bridge the gap between timeseries and natural language. 

\item Leveraging the periodicity of timeseries, our group attention mechanism reduces the time and space complexity of the self-attention mechanism with accuracy guarantees, allowing  \system to scale to long timeseries data.

\item Guided by an approximation error bound, our adaptive scheduler dynamically adapts the number of groups and the batch size to the distribution properties of the evolving feature embeddings, making group attention efficient and easily tuning.

\item We conduct experiments on various datasets and different analytics tasks, confirming that \system is up to 63 times faster than the state-of-the-art, yet better in accuracy. 

\end{compactitem}

